Constraint-Guided Prediction Refinement via Deterministic Diffusion Trajectories

Many real-world machine learning tasks require outputs that satisfy hard constraints, such as physical conservation laws, structured dependencies in graphs, or column-level relationships in tabular data. Existing approaches rely either on domain-specific architectures and losses or on strong assumptions on the constraint space, restricting their applicability to linear or convex constraints. We propose a general-purpose framework for constraint-aware refinement that leverages denoising diffusion implicit models (DDIMs). Starting from a coarse prediction, our method iteratively refines it through a deterministic diffusion trajectory guided by a learned prior and augmented by constraint gradient corrections. The approach accommodates a wide class of non-convex and nonlinear equality constraints and can be applied post hoc to any base model. We demonstrate the method in two representative domains: constrained adversarial attack generation on tabular data with column-level dependencies and in AC power flow prediction under Kirchhoff's laws. Across both settings, our diffusion-guided refinement improves both constraint satisfaction and performance while remaining lightweight and model-agnostic.

==> old_theorems.tex <==
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}

\section{Summary}
In this work, we propose a hybrid approach to improve the physical plausibility of predictions made by a base neural network estimator. Our method leverages a conditional diffusion model trained on residuals, defined as the difference between the true target and the prediction of the base model, to stochastically correct the initial estimate. The diffusion model learns a distribution over physically meaningful corrections, effectively refining predictions toward the constraint manifold defined by domain-specific physical equations (e.g., conservation laws, Kirchhoff's laws).

We formalize this as a two-stage framework: first, a base model $f_\theta$ provides an initial approximation; then, a diffusion model $D_\phi$ samples residuals $r$ such that the corrected output $\hat{y} = f_\theta(x) + r$ becomes both accurate and compliant with physical constraints. To enforce this, the diffusion model is trained with a composite loss that balances data fidelity and constraint satisfaction. We show theoretically that, in the limit where constraint regularization dominates, the output distribution of the corrected predictions converges (in probability and weakly) to the physical manifold. This provides a principled, probabilistic mechanism for projecting approximate neural predictions onto the manifold of physically feasible solutions.


\begin{theorem}[First-Order Residual Correction Toward the Physics Manifold]
Let $\mathcal{F} : \mathbb{R}^d \rightarrow \mathbb{R}^k$ be a differentiable function defining the physical constraints, and let
\[
\mathcal{M} := \{ y \in \mathbb{R}^d \mid \mathcal{F}(y) = 0 \}
\]
be the corresponding physical (constraint) manifold. Let $f_\theta(x) \in \mathbb{R}^d$ be a base model prediction for input $x$, such that $f_\theta(x) \notin \mathcal{M}$ but is close to it. Suppose there exists a residual vector $r \in \mathbb{R}^d$ such that $f_\theta(x) + r \in \mathcal{M}$.

Then, to first order, the residual that restores physical consistency can be approximated by
\[
r \approx -J_{\mathcal{F}}(f_\theta(x))^\dagger \mathcal{F}(f_\theta(x)),
\]
where $J_{\mathcal{F}}(f_\theta(x)) \in \mathbb{R}^{k \times d}$ is the Jacobian of $\mathcal{F}$ evaluated at $f_\theta(x)$, and $^\dagger$ denotes the Moore–Penrose pseudoinverse.
\end{theorem}

\begin{proof}
Since $\mathcal{F}$ is differentiable at $f_\theta(x)$, we apply the first-order Taylor expansion of $\mathcal{F}$ at $f_\theta(x)$:
\[
\mathcal{F}(f_\theta(x) + r) \approx \mathcal{F}(f_\theta(x)) + J_{\mathcal{F}}(f_\theta(x)) r.
\]
We want the corrected prediction $f_\theta(x) + r$ to satisfy the physical constraint:
\[
\mathcal{F}(f_\theta(x) + r) = 0.
\]
Substituting the (first order) Taylor expansion into this condition gives:
\[
\mathcal{F}(f_\theta(x)) + J_{\mathcal{F}}(f_\theta(x)) r \approx 0.
\]
Rearranging the terms we get:
\[
J_{\mathcal{F}}(f_\theta(x)) r = -\mathcal{F}(f_\theta(x)).
\]
The least norm solution for this linear system is given by the Moore–Penrose pseudoinverse:
\[
r = -J_{\mathcal{F}}(f_\theta(x))^\dagger \mathcal{F}(f_\theta(x)).
\]
This expression gives a first-order approximation to the residual that projects $f_\theta(x)$ onto the constraint manifold $\mathcal{M}$.
\end{proof}


\paragraph{Theorem 2: Diffusion Sampling as Approximate Stochastic Projection onto a Constraint Manifold}

\begin{definition}[Physics Manifold]
Let $\mathcal{F} : \mathbb{R}^d \rightarrow \mathbb{R}^k$ be a continuously differentiable function defining the physical constraints. The physical (or constraint) manifold is defined as
\[
\mathcal{M} := \{ y \in \mathbb{R}^d \mid \mathcal{F}(y) = 0 \}.
\]
\end{definition}

\begin{definition}[Residual Diffusion Model]
Let $f_\theta(x) \in \mathbb{R}^d$ be a base estimator, and let $D_\phi(r \mid f_\theta(x))$ denote a conditional diffusion model trained to generate residuals $r$ such that the corrected prediction $\hat{y} := f_\theta(x) + r$ is both accurate and physically valid.
\end{definition}

\begin{theorem}[Stochastic Projection in the Infinite Constraint Limit]
Let $\mathcal{F}$ be Lipschitz continuous, and assume for each $\lambda > 0$, the diffusion model $D_{\phi_\lambda}$ is trained to minimize the expected loss:
\[
\mathcal{L}_\lambda(\phi) := \mathbb{E}_{x, y} \left[ \mathbb{E}_{r \sim D_\phi(\cdot \mid f_\theta(x))} \left( \| f_\theta(x) + r - y \|^2 + \lambda \| \mathcal{F}(f_\theta(x) + r) \|^2 \right) \right].
\]
Suppose:
\begin{enumerate}
    \item The support of $D_{\phi_\lambda^*}(\cdot \mid f_\theta(x))$ is contained in a compact set $K \subset \mathbb{R}^d$, for all $x$ and $\lambda$.
    \item $\mathcal{F}$ is Lipschitz continuous on $K$.
\end{enumerate}
Then, for any $\varepsilon > 0$,
\[
\lim_{\lambda \to \infty} \mathbb{P}_{r \sim D_{\phi_\lambda^*}(\cdot \mid f_\theta(x))} \left[ \| \mathcal{F}(f_\theta(x) + r) \| \leq \varepsilon \right] = 1.
\]
That is, the corrected prediction $\hat{y} = f_\theta(x) + r$ converges in probability to the constraint manifold $\mathcal{M}$ as $\lambda \to \infty$.
\end{theorem}

\begin{proof}
Let $S_\varepsilon := \{ r \in \mathbb{R}^d \mid \| \mathcal{F}(f_\theta(x) + r) \| \leq \varepsilon \}$.

Suppose by contradiction that the result does not hold. Then there exist constants $\varepsilon > 0$, $\delta > 0$, and a sequence $\lambda_n \to \infty$ such that
\[
\mathbb{P}_{r \sim D_{\phi_{\lambda_n}^*}(\cdot \mid f_\theta(x))} \left[ \| \mathcal{F}(f_\theta(x) + r) \| > \varepsilon \right] \geq \delta \quad \text{for all } n.
\]
Denote $A := \{ r \in \mathbb{R}^d \mid \| \mathcal{F}(f_\theta(x) + r) \| > \varepsilon \}$. Then,
\[
\mathbb{E}_{r \sim D_{\phi_{\lambda_n}^*}} \left[ \| \mathcal{F}(f_\theta(x) + r) \|^2 \right] \geq \int_{A} \| \mathcal{F}(f_\theta(x) + r) \|^2 \, dD_{\phi_{\lambda_n}^*}(r) > \varepsilon^2 \delta.
\]
Thus, the total training loss satisfies:
\[
\mathcal{L}_{\lambda_n}(\phi_{\lambda_n}^*) \geq \text{MSE} + \lambda_n \cdot \varepsilon^2 \delta \to \infty \quad \text{as } n \to \infty.
\]
But this contradicts the assumption that $\phi_{\lambda_n}^*$ minimizes $\mathcal{L}_{\lambda_n}(\phi)$ over $\phi$; one could trivially assign all probability mass to points $r$ such that $f_\theta(x) + r \in \mathcal{M}$, driving the physics penalty to zero.

Therefore, for all $\varepsilon > 0$,
\[
\lim_{\lambda \to \infty} \mathbb{P} \left[ \| \mathcal{F}(f_\theta(x) + r) \| \leq \varepsilon \right] = 1.
\]
\end{proof}

\begin{remark}[Stochastic Projection]
The result implies that the distribution of corrected predictions
\[
\hat{y} = f_\theta(x) + r, \quad r \sim D_{\phi_\lambda^*}(\cdot \mid f_\theta(x)),
\]
acts as a \textit{stochastic projection operator} onto the manifold $\mathcal{M}$ in the limit $\lambda \to \infty$. That is,
\[
\hat{y} \sim \Pi_{\mathcal{M}}^{\text{stoch}}(f_\theta(x)),
\]
where $\Pi_{\mathcal{M}}^{\text{stoch}}$ denotes a random mapping approximating a projection onto the constraint manifold.
\end{remark}

\paragraph*{Extensions and Interpretations}

\paragraph*{(a) Weak Convergence of Output Distributions}
Let $\mu_\lambda := \text{Law}(f_\theta(x) + r)$, where $r \sim D_{\phi_\lambda^*}(\cdot \mid f_\theta(x))$. Then $\mu_\lambda$ is a sequence of probability measures on a compact set $K \subset \mathbb{R}^d$.

By Prokhorov’s theorem, $\{ \mu_\lambda \}$ is tight. The previous theorem implies that for any open neighborhood $\mathcal{M}_\varepsilon := \{ y \in \mathbb{R}^d \mid \| \mathcal{F}(y) \| \leq \varepsilon \}$,
\[
\mu_\lambda(\mathcal{M}_\varepsilon) \to 1 \quad \text{as } \lambda \to \infty.
\]
Therefore, $\mu_\lambda \xrightarrow{w} \mu_\infty$, where $\text{supp}(\mu_\infty) \subseteq \mathcal{M}$.

\begin{remark}
This result shows that the diffusion model defines a sequence of distributions converging weakly to a measure supported on the manifold $\mathcal{M}$.
\end{remark}

\paragraph*{(b) Bayesian Interpretation}
Assume a generative model:
\begin{align*}
    y \mid r, x &\sim \mathcal{N}(f_\theta(x) + r, \sigma^2 I), \\
    p(r \mid x) &\propto \exp\left( -\frac{\lambda}{2} \| \mathcal{F}(f_\theta(x) + r) \|^2 \right).
\end{align*}

Then the posterior over $r$ is:
\[
p(r \mid x, y) \propto \exp\left( -\frac{1}{2\sigma^2} \| y - (f_\theta(x) + r) \|^2 - \frac{\lambda}{2} \| \mathcal{F}(f_\theta(x) + r) \|^2 \right).
\]

\begin{remark}
The diffusion model $D_\phi(\cdot \mid f_\theta(x))$ may be viewed as an amortized sampler approximating the posterior $p(r \mid x, y)$. As $\lambda \to \infty$, the posterior concentrates on values of $r$ such that $f_\theta(x) + r \in \mathcal{M}$, yielding physics-consistent predictions.
\end{remark}

